Predict and Match: Prophet Inequalities with Uncertain Supply

We consider the problem of selling perishable items to a stream of buyers in order to maximize social welfare. A seller starts with a set of identical items, and each arriving buyer wants any one item, and has a valuation drawn i.i.d. from a known distribution. Each item, however, disappears after an a priori unknown amount of time that we term the horizon for that item. The seller knows the (possibly different) distribution of the horizon for each item, but not its realization till the item actually disappears. As with the classic prophet inequalities, the goal is to design an online pricing scheme that competes with the prophet that knows the horizon and extracts full social surplus (or welfare). Our main results are for the setting where items have independent horizon distributions satisfying the monotone-hazard-rate (MHR) condition. Here, for any number of items, we achieve a constant-competitive bound via a conceptually simple policy that balances the rate at which buyers are accepted with the rate at which items are removed from the system. We implement this policy via a novel technique of matching via probabilistically simulating departures of the items at future times. Moreover, for a single item and MHR horizon distribution with mean $\mu$, we show a tight result: There is a fixed pricing scheme that has competitive ratio at most $2 - 1/\mu$, and this is the best achievable in this class. We further show that our results are best possible. First, we show that the competitive ratio is unbounded without the MHR assumption even for one item. Further, even when the horizon distributions are i.i.d. MHR and the number of items becomes large, the competitive ratio of any policy is lower bounded by a constant greater than $1$, which is in sharp contrast to the setting with identical deterministic horizons.

==> DP-constant.tex <==
\paragraph{Competing with {\sc VPro}.}
\label{sec:DPConst}
In this section, we consider the following more general setting: There are $m$ items and the horizon of item $i$ is drawn from an arbitrary horizon distribution $H_i$. There are $n$ unit-demand buyers and the value of the $h$-th arriving buyer for any of the items is drawn from value distribution $V_h$.\footnote{We can easily generalize this to the setting where the buyers have different valuations for different items.} Note that we know the arrival order of buyers. Since we already observed that competing with the omniscient prophet is impossible in this setting, we consider a weaker benchmark and show that in this setting we can achieve a constant fraction of $\textsc{VPro}$. In the rest of this section, we use prophet to refer to \textsc{VPro}. 
  
We first find an upper bound for $\textsc{VPro}$. Let $X_h$ and $Z_i$ be random variables with distribution $V_h$ and $H_i$, respectively. Consider the following LP: 
\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum_{v,h,i} y_{ivh} \cdot \Pr[Z_i \ge h] \cdot v &\\
\text{subject to}& \displaystyle\sum_i  y_{ivh} \cdot \Pr[Z_i \ge h]  \le \Pr[X_h = v],\quad&\forall h,v,\\
& \displaystyle\sum_{v,h} y_{ivh} \le 1, \quad& \forall i.
\end{array}
\end{equation*}
Variable $y_{ivh}$ is the probability that $h$-th buyer is assigned to item $i$ and its value is $v$, given that the horizon of item $i$ is not less than $h$. Note that based on this definition $y_{ivh} \le \Pr[X_h=v]$ which can be encoded as a set of constraints in LP.  We show the above LP is a constant-factor relaxation to {\sc VPro}. This is not obvious is because of the final constraint where the $y$ variable is not discounted by the probability the item survives.  The main idea builds on the work by Samuel-Cahn~\cite{samuel1996optimal}. It shows for a single item, the presence of a stochastic horizon is equivalent to discounting the value in terms of the optimal dynamic programming solution. We show that this observation holds even for an LP relaxation: Since the policy {\sc VPro} does not know when the items depart, at time $h$, its decision to assign buyers to items cannot depend on departure times in the future.
\begin{lemma} (Proved in Appendix~\ref{app:VPRO-LP})
	\label{lem:VPRO-LP}
	The value $\textsc{Opt}$ of the above LP is at least $\textsc{VPro}$.
\end{lemma} 

We next present an algorithm, shown below, in which we assume the $h$-th arriving buyer tells us her true value.  In Appendix~\ref{app:pricingScheme}, we also present a pricing scheme implementation of the algorithm which is incentive compatible. %The algorithm is shown below:

\begin{figure}[htbp]
\center
\noindent\fbox{%
	\parbox{0.95\textwidth}{%
When the $h$-th buyer announces value $v$: 
\begin{itemize}
	\item Create set $S_{hv}$: insert each item $i$ independently in $S_{hv}$ with probability $\frac{y_{ivh}}{2 \Pr[X_h=v]}$.
	\item Consider an arbitrary order of items in $S_{hv}$ and assign the buyer to the first item $i$ such that the horizon of $i$ is at least $h$ and $i$ has not been assigned in previous steps. 
\end{itemize}
}%
}
\end{figure}

\begin{theorem} (Proved in Appendix~\ref{app:DPConst})
	\label{thm:DPConst}
	 Let $\textsc{Alg}$ denote the welfare of the algorithm described above. Then, $8 \textsc{Alg} \ge \textsc{VPro}$.
\end{theorem}     

%In , we present a \emph{truthful} pricing implementation of the above algorithm. 


==> DP.tex <==
\section{Competing with the Dynamic Programming Benchmark}
\label{sec:DP}
\label{sec:non-iid-Hard}
So far, we have shown that for the setting with multiple identical items with {\em i.i.d.} MHR horizons and a stream of {\em i.i.d.}-valuation buyers, there is a constant approximation of the omniscient prophet's welfare ($\textsc{Pro}$). In this section, we seek to relax these two assumptions. As we have already seen in Theorem~\ref{thm:gen_low_any}, when there is a general horizon distribution, achieving a constant approximation of $\textsc{Pro}$ is not possible even with {\em i.i.d.} buyers. In this section, we show that the {\em i.i.d.} condition on values of buyers also cannot be relaxed much when the goal is to achieve welfare that is a constant fraction of $\textsc{Pro}$. Then, we consider the weaker benchmark $\textsc{VPro}$ (see Definition~\ref{def:proph}) where we compete against a solution that knows the buyer values but not the horizons of the items. We show that we can achieve a constant approximation to this benchmark in a fairly general setting. %where the horizon of item $i$ is drawn from an arbitrary horizon distribution $H_i$ and the value of the $j$-th arriving buyer is drawn from distribution $V_j$. 

\input{non-iid-lowerBound.tex}
\input{DP-constant.tex} 


==> constLowRate.tex <==
\subsection{$2$-Competitive Dynamic Pricing Scheme: Proof of Theorem~\ref{thm:ubone}} 
\label{sec:geo2Approx}
In this section, we show that the lower bound of $2$ is tight for low-rate geometric horizons by showing that the dynamic pricing scheme that balances the rate of departure of sellers with the rate of matching buyers is $2$-competitive. We will achieve this by developing a closed form upper bound for {\sc Pro}' based on an LP relaxation. The crucial insight for developing the closed form bound is noting that if $T_k$ denotes the (random amount of) time the process spends in state $k$, then $\E[T_k]$ is monotonically decreasing in $k$. We will subsequently show that the dynamic pricing scheme effectively couples with this LP bound, but executes at twice the speed.  We will build on this idea when we develop a policy for general MHR distributions in the next section.

\subsubsection{LP Relaxation for {\sc Pro}' } In the LP relaxation for {\sc Pro'},  $n_k(v)$ denotes the expected number of buyers with value $v$ matched by the prophet when in state $k$.
\begin{equation*}
\label{LP:ProLowGeo} 
\begin{array}{ll@{}ll}
\text{maximize}   & \displaystyle \sum_{v} \sum_{k=1}^m n_k(v) \cdot v &\\
\text{subject to} & \displaystyle  \sum_{v, k' \le k} n_{k'}(v) \le k , \quad&\forall k, \\
& \displaystyle n_k(v) \leq \E[T_k]\Pr_{X \sim V}[X = v], \quad&\forall v, k.
\end{array}
%\label{equation:lp}
\end{equation*}  
The first set of constraints states that the expected number of buyers matched after arriving after entering state $k$ is not more than the total number of remaining items (which is $k$). The second set of constraints states that the expected number of items of value $v$ matched in state $k$ is at most the expected time spent in state $k$ times the per-step probability of observing the value $v$.  We now show that this LP has a closed form upper bound.  
 \begin{lemma} 
 	\label{lem:ProLowRate}
	 	$\textsc{Pro}' \leq   \sum_{k}  \E_{X \sim V}[X \mid X \geq p_k]$ where $p_k$ satisfies $\Pr_{X \sim V}[X \ge p_k]= \frac{1}{\E[T_k]}$  
 \end{lemma}
\begin{proof}
	Let $\lambda_k$ be the Lagrange multiplier associated with the first set of constraints for any $k$. The partial Lagrangian of the LP is: 
	\begin{align*}
		\mathcal{L}(\Vec{\lambda}) =& \sum_{k,v} n_k(v) \cdot v + \sum_k \lambda_k \left (k -\sum_{v,k' \le k} n_{k'}(v) \right)  =   \sum_{k,v} n_k(v) \left (v - \sum_{k \le k'}  \lambda_{k'} \right) + \sum_k \lambda_k k, \\
		&n_k(v) \leq E[T_k]\Pr_{X \sim V}[X = v], \quad\forall v, k.
	\end{align*}
	
	Let $p_k= \sum_{k \le k'} \lambda_{k'}$. The partial Lagrangian is maximized when $n_k(v)= E[T_k] \Pr_{X \sim V}[X = v]$ if $v \ge p_k$ and $n_k(v)=0$ otherwise. Therefore, we can get the following upper bound for any $\Vec{\lambda}$: 
	\begin{align*}
		\textsc{Pro}' &\leq  \sum_{k,v \ge p_k}E[T_k] \Pr_{X \sim V}[X = v] \cdot v + \sum_k \lambda_k \left (k - \sum_{k' \le k} \sum_{v \ge p_{k'}}E[T_{k'}]\Pr_{X \sim V}[X = v] \right) \\
		& =   \sum_{k,v \ge p_k}E[T_k] \Pr_{X \sim V}[X = v] \cdot v + \sum_k \lambda_k \left (k - \sum_{k' \le k}E[T_{k'}]\Pr_{X \sim V}[X \ge p_{k'}] \right). \numberthis \label{eq:UpPRoLow}
	\end{align*}
	We claim that we can always set $\Vec{\lambda}$ in a way that for each $k$ the following holds: 
	\begin{equation}
	\label{eq:lagProLow}
	\sum_{k' \le k} E[T_{k'}]\Pr_{X \sim V}[X \ge p_{k'}] = k.
	\end{equation}
	The above equation is equivalent to the following for any $k$:
	\begin{equation}
	\label{eq:lagPro2Low}
	\Pr_{X \sim V}[X \ge p_k]= \frac{1}{E[T_k]} 
	\end{equation}  
	Note that $ {E[T_k]} \ge 1$ and the only constraint in setting $p_k$ is that it should be decreasing in $k$ because Lagrange multipliers are non-negative. Since ${E[T_k]}$ is increasing in $k$, we can guarantee that $\Vec{\lambda}$ can be set in a way that for each $k$, Equation~(\ref{eq:lagProLow}) holds.   
	
	Now using Equations~(\ref{eq:UpPRoLow}), (\ref{eq:lagProLow}), and~(\ref{eq:lagPro2Low}), we get the following upper bound for $\textsc{Pro}'$:  
	\begin{equation}
	\label{eq:URProLow}
	\textsc{Pro}' \leq  \sum_{k} \sum_{v \geq p_k} {E[T_k]} v \cdot \Pr_{X \sim V}[X = v] =  \sum_{k}  \E_{X \sim V}[X \mid X \geq p_k]. \qedhere
	\end{equation}
	\end{proof}
	

\subsubsection{Analysis of Dynamic Pricing Scheme.} Recall that the dynamic pricing scheme will match the rate of departure of sellers with the rate of acceptance of buyers. It can do this by posting the price $p_k$ when there are $k$ items left. This is equivalent to set $\beta_k=1$ in $\textsc{Alg}'$, and would cause the policy to transition from state $k$ to state $k-1$ at rate $2 k \lambda_k$, {\em i.e.}, twice the rate of transition in our upper bound for {\sc Pro'}.  Since the state transitions with equal probability due to a departure or due to a matching, we have: 
\[
\E[\textsc{Alg}'] = \frac{1}{2} \sum_{k}  \E_{X \sim V}[X \mid X \geq p_k].
\]
Combined with Lemma~\ref{lem:ProLowRate}, this policy is a $2$-competitive, completing the proof of Theorem~\ref{thm:ubone}.



==> non-iid-lowerBound.tex <==
\paragraph{Lower Bounds for Non-\emph{I.I.D.} Buyers.} 	
In Appendix~\ref{app:eg}, we present two simple examples with non-{\em i.i.d.} buyers and a single item with MHR horizon. We show that in neither of these settings, a constant approximation of $\textsc{Pro}$ is possible. In the first example (Example~\ref{eg1}) buyer valuations are deterministic, the arrival order is known, and the horizon is MHR, and in the second example (Example~\ref{eg2}), buyer valuations are deterministic, the arrival is according to a known distribution of permutations, and the horizon is deterministic.  Note that when the deterministic horizon equals the number of buyers, a $2$-approximation is possible even when the valuations are non-{\em i.i.d.} and arrival order of buyers is adversarial. %Note that when the buyers are {\em i.i.d.}, any fixed horizon $n$ is equivalent with the classic prophet inequality with $n$ {\em i.i.d.} buyers. 
However,  for non-{\em i.i.d.} buyers (even with deterministic values), having a smaller horizon precludes a constant-competitive algorithm.  

\iffalse
In the first example, buyer valuations are deterministic and known, and the horizon is MHR. Note that in this setting the order of arrival is also known to the algorithm. The following example shows that no algorithm can be a constant approximation of $\textsc{Pro}$.   
\begin{example}
\laebl{eg1}
%There is a family of instances when the $h$-th arriving buyer has known value $v_h$, and the horizon distribution $H$ is MHR such that no algorithm can achieve a constant fraction of $\textsc{Pro}$.
%\end{theorem}
%\begin{proof}
Let the horizon distribution be the geometric distribution with parameter $0.5$. Consider a set of $n$ buyers such that  $v_h=2^h$. The expected value of the prophet is $\Theta(n)$ while any algorithm can only achieves a constant value in expectation.
%\end{proof}
\end{example}

In the second example, there are $k$ buyers, and their valuations are deterministic. The arrival is according to a known distribution of permutations. We show that no algorithm can get a constant approximation even if the horizon is a fixed and known to be $n \leq k$. 
\begin{example}
\label{eg2}
Let $k=2(n-1)+1$ and $v_j= 2^{j+1}$ if $j < n$ and $v_j=0$ otherwise. The arrival order of buyers is one of the following $k+1$ permutations: For $1 \le i \le n-1$, permutation $\pi_i = \left(1,2, \dots i, n, n+1, \ldots, k, i+1, \ldots, n-1 \right)$ is chosen with probability $\frac{1}{2^i}$ and permutation $\pi_{n}= \left(n, n+1, \ldots, k, 1,2,\ldots n-1 \right)$ is chosen with probability $\frac{1}{2^{n-1}}$. 

Any policy can only generate O(1) in expectation while the value of the prophet is $\Theta(n)$. Note that this is tight because randomly picking one of the first $n$ buyers is a $\Theta(n)$-approximation.  
\end{example}


Note that the deterministic horizon is the simplest horizon distribution and for $k = n$ this is the classic prophet inequality and $2$-approximation is possible even when the valuations are non-{\em i.i.d.} and arrival order of buyers is adversarial. %Note that when the buyers are {\em i.i.d.}, any fixed horizon $n$ is equivalent with the classic prophet inequality with $n$ {\em i.i.d.} buyers. 
However,  for non-{\em i.i.d.} buyers (even with deterministic values), having a small horizon precludes a constant-competitive algorithm.  \fi

%\begin{theorem}
%	There exists a family of instances where there are $k$ buyers with deterministic valuations whose arrival order is drawn from a known distribution, such that no policy is an $o(n)$-approximation of the prophet's value where $n$ is the fixed known horizon. 
%\end{theorem}





==> prelim.tex <==
\section{Preliminaries}
\label{sec:single}
There are $m$ items, where item $i$ has its horizon drawn from distribution $H_i$. An infinite stream of unit-demand buyers arrive and the valuation of the $h$-th arriving buyer is a random variable $X_h$ which is drawn independently from the common value distribution $V$. An online policy knows whether an item exists at the current time step, and only has conditional distributional knowledge of when the item will depart, {\em i.e.}, at time $h$, the policy can calculate the distribution $H_i \mid H_i \ge h$. It can only assign an item to a buyer if the item has not departed by the current time step, and in this case, any such item can be feasibly assigned to the buyer. 

\iffalse
Note that the assumption that there is an infinite stream of buyers is without loss of generality because we can encode an upper bound on the number of buyers in the distribution $H$. Further note that the setting where $H$ is deterministic corresponds to the classic prophet inequality setting studied by Hill and Kertz~\cite{hill1982comparisons}.

First, we define the omniscient prophet and two other less powerful prophets, and state a simple proposition for the single-item setting. 
\begin{definition}
	\rm
	\label{def:proph}
	Define $\textsc{Pro}$ to be the expected welfare of the omniscient prophet who knows both the realized valuations and horizon. Let $\textsc{VPro}$ be the welfare of the valuation prophet who only knows the realized valuations but not the realized horizon.
	Finally, the horizon prophet who knows the realized horizon but not the realized values, and its welfare is denoted by $\textsc{HPro}$.
\end{definition}
The different types of prophets in definition~\ref{def:proph} can be defined similarly when there are multiple items (Section~\ref{sec:multi}) with stochastic horizons and we use the same notation for that problem.
\fi

Define $\textsc{Pro}$ to be the expected welfare of the omniscient prophet who knows both the realized valuations and horizon. The goal is to design an online pricing scheme (or more generally, an incentive-compatible online mechanism) whose welfare is competitive with that of the prophet. We use {\sc Alg} to denote the expected welfare of a policy that knows $H_i$'s and $V$, but not the respective realizations and {\sc Alg*} is the optimal among such policies. In the rest of the paper, without creating ambiguity, we slightly abuse the notations $\textsc{Pro}$/{\sc Alg} %(similarly $\textsc{VPro}$, $\textsc{HPro}$, $\textsc{Alg}$)
 to refer to both the prophet/algorithm and the expected welfare achieved by the prophet/algorithm.

\iffalse
We have the following immediate observations for the single-item setting; their proofs follow from similar results for the classic prophet inequality~\cite{samuel1996optimal}.
\begin{prop}
	\label{prop:alg_vpro}
	\label{prop:tpro_pro}
	$\textsc{Alg*} \leq \textsc{VPro} \leq 2\textsc{Alg*}$ and $\textsc{HPro} \leq \textsc{Pro} \leq 2\textsc{HPro}$.
\end{prop}
%\begin{proof}
%	It's similar to the classic prophet inequality and is discussed in \cite{samuel1996optimal}.
%\end{proof}

%\begin{prop}
%	$\textsc{HPro} \leq \textsc{Pro} \leq 2\textsc{HPro}$. 
%\end{prop}
%\begin{proof}
%	The inequality holds for any realized horizon because of the classic prophet inequality.
%\end{proof}   
\fi

\input{single_general}

\paragraph{Monotone-Hazard-Rate (MHR) Horizon Distributions.} Given the above lower bound, we restrict the horizon distributions $H_i$ to satisfy the monotone-hazard-rate (MHR) condition. Several distributions satisfy the MHR condition, including uniform, geometric, deterministic, and Poisson. 

\begin{definition}
\rm
A horizon distribution $H$ satisfies the MHR condition if for all $h^* \ge 1$, we have:
$$\Pr_{h \sim H}[h \geq h^* + 2 \mid h \geq h^* + 1] \leq \Pr_{h \sim H}[h \geq h^* + 1 \mid h \geq h^*],$$
{\em i.e.}, the process is more and more likely to stop as time goes on.
\end{definition}

The example below shows that even with MHR distributions, the assumption that buyer valuations are \emph{i.i.d.} is necessary --- indeed, no constant-competitive algorithm is possible for one item, even in the setting where buyer valuations are deterministic with known order of arrival. 

\begin{example}
\label{eg1}
There is $m=1$ item with horizon following the geometric distribution with parameter $0.5$. Consider a set of $n$ buyers such that  $v_h=2^h$ for $h = 1,2,\ldots,n$. The expected value of the prophet is $\Theta(n)$ while any algorithm can only achieves a constant value in expectation.
\end{example}





==> single.tex <==
\input{single_MHR}



==> single_general.tex <==
% !TEX root = ms.tex
\paragraph{General Horizon Distributions.}
\label{sec:singleGen} 
First, we consider the general case where there is no restriction on the horizon distribution. We show  that in this case, %the value prophet $\textsc{VPro}$ cannot compete with the omniscient prophet $\textsc{Pro}$. Combining with Proposition~\ref{prop:alg_vpro}, this implies that
even when the buyer valuations are {\em i.i.d.}, and regardless of whether the algorithm knows the realized valuations, not knowing the realized horizon severely limits achievable welfare. 

%To characterize the lower bound, we assume the time horizon is at most $n$.
\begin{theorem} (Proved in Appendix~\ref{app:gen_low_any})
\label{thm:gen_low_any}
For any $m \ge 1$ items, there exists a family of instances such that $\textsc{Pro}$ has welfare $\Omega\left(\frac{\log n}{\log \log n}\right)$-factor larger than any  online policy, even if the policy knows all the realized values, but not the realized horizons. Here,  $n = \max_i \{\mathrm{supp}(H_i)\}$. %\cdot \textsc{Alg^*}$ where $n = \max \{\mathrm{supp}(H)\}$. 
%This lower bound is almost matched by a fixed pricing scheme that is $O\left(\log n\right)$-competitive.  Moreover, any fixed-pricing is $\Omega\left(\log n\right)$-competitive
\end{theorem}

\iffalse 
\begin{theorem}
\label{thm:gen_upp_sin}
The approximation ratio for any single-threshold algorithm without information of realized horizon is $\Omega\left(\log n\right)$ again the prophet $\textsc{Pro}$. 


\end{theorem}
\begin{proof}
Consider the same horizon and valuation distributions as the ones in the proof of Theorem \ref{thm:gen_low_any}, but instead of setting $c = \log_2 k$, we set $c$ to be a constant greater than $1$. Let $\textsc{Sing}$ be the optimal single-threshold algorithm with information of realized valuations but not realized horizon. We have
\begin{align*}
\textsc{Sing} &= \max_{i = 1}^{ck} \left\{\E[v_1 \mid v_1 \geq a_i] \cdot \sum_j \pi_j \cdot \Pr_{v_1, \ldots, v_n}[M_j \geq a_i]\right\}\\
&\leq \max_{i = 1}^{ck} \left\{\frac{1}{1 - {2^{c^{-1}-1}}} \cdot a_i \cdot \sum_j \pi_j \cdot \Pr_{v_1, \ldots, v_n}[M_j \geq a_i]\right\}\\
&\leq \frac{1}{1 - {2^{c^{-1}-1}}} \cdot \max_{i = 1}^{ck} \left\{2^{i/c} \cdot \sum_j 2^{-j} \cdot \Pr_{v_1, \ldots, v_n}[M_j \geq 2^{i/c}]\right\}\\
&\leq \frac{1}{1 - {2^{c^{-1}-1}}} \cdot \max_{i = 1}^{ck} \left\{2^{i/c} \cdot \sum_j 2^{-j} \cdot \min\left(1, 2^{cj-i+1}\right)\right\}\\
&\leq \frac{1}{1 - {2^{c^{-1}-1}}} \cdot \max_{i = 1}^{ck} \left\{2^{i/c} \cdot 2^{-(i - 1)/c} \cdot \left(5 + \frac{1}{2^{c-1} - 1}\right)\right\}\\
&= O(1).
\end{align*}

On the other hand, we still have $\textsc{Pro} = \Omega(k)$. As $n = 2^{ck}$, this shows an $\Omega(\log n)$ gap.
\end{proof}

\fi 

%\begin{theorem}
%In the general departure setting, there is an $O\left(\min(m, \log n)\right)$-approximation single-threshold algorithm without information of realized valuations or realized departure time.
%\end{theorem}
%\begin{proof}
%An algorithm can set the price at each $a_i$ in the support of the valuation distribution and get welfare at least $a_i \Pr[\text{The seller saw a value }\geq a_i]$, summing over $i$, we have
%\begin{align*}
%\sum_i a_i \Pr[\text{The seller saw a value }\geq a_i] \geq \sum_i (a_i - a_{i - 1}) \Pr[\text{The seller saw a value }\geq a_i] = \textsc{Opt}.
%\end{align*}
%
%An algorithm can pretend the seller departs right after $2^k$ steps for $k = 0, 1, \ldots, \lceil\log_2 n\rceil$.
%
%\end{proof}

%\begin{theorem}
%In the general departure setting with $n$ non-{\em i.i.d.} buyers and random ordering, in polynomial time we can approximate the optimal algorithm which can see the identities of previous buyers within a multiplicative constant.
%\end{theorem}
%\begin{proof}
%Without loss of generality, assume $n$ is even. Let $\textsc{First}$ be the optimal welfare that can be drawn by a non-clairvoyant algorithm in the first $n/2$ steps, and $\textsc{Last}$ be the optimal welfare that can be drawn by a non-clairvoyant algorithm in the last $n/2$ steps. We know the optimal algorithm satisfies $\textsc{Alg} \leq \textsc{First} + \textsc{Last}$ as the RHS allows the algorithm to choose at most $2$ buyers. We also have
%\begin{align*}
%2\textcolor{red}{\text{or other const}}\textsc{First} \geq p \cdot \textsc{ProHalf} \geq \textsc{Last}
%\end{align*}
%where $p$ is the probability that the seller didn't depart in the first $n/2$ steps, and $\textsc{ProHalf}$ is the welfare drawn by the prophet if the seller always depart right after $n/2$ steps. Therefore, $\textsc{Alg} \leq 3\textsc{First}$.
%
%Let $F_i(x)$ be the cumulative distribution function (CDF) for the valuation distribution $V_i$ of the $i$-th buyer. Define a new valuation distribution $V$ whose CDF $F(x)$ is defined as: $F(x) := \sum_{i = 1}^n \frac{1}{n}F_i(x)$. If the buyers are independently drawn from $V$, the optimal algorithm for the first $n/2$ steps --- $\textsc{First}'$ ---  will be a simple dynamic programming problem computable in polynomial time. Slightly abusing notations, we use $\textsc{First}$ and $\textsc{First}'$ to denote the corresponding dynamic programming policies. We have
%\begin{align*}
%\textstyle\textsc{First}'(\bigtimes_{i = 1}^n V_i) \geq \textsc{First}'(V^n) \geq \textsc{First}(V^n) \geq \frac{1}{2} \textsc{First}(\bigtimes_{i = 1}^n V_i).
%\end{align*}
%The second inequality comes from the fact that $\textsc{First}'$ is the optimal algorithm for $V^n$. We will state and prove the other inequalities above as lemmas:
%\begin{lemma}
%$\textsc{First}'(\bigtimes_{i = 1}^n V_i) \geq \textsc{First}'(V^n)$.
%\end{lemma}
%\begin{proof}
%
%
%\end{proof}
%\begin{lemma}
%$\textsc{First}(V^n) \geq \frac{1}{2} \textsc{First}(\bigtimes_{i = 1}^n V_i)$.
%\end{lemma}
%\begin{proof}
%
%
%\end{proof}
%Therefore, $\textsc{First}(\bigtimes_{i = 1}^n V_i) \geq \frac{1}{6} \textsc{Alg}$.
%\end{proof}

